Reasoning about disclosure in data integration in the presence of source constraints

Data integration systems allow users to access data sitting in multiple sources by means of queries over a global schema, related to the sources via mappings. Data sources often contain sensitive information, and thus an analysis is needed to verify that a schema satisfies a privacy policy, given as a set of queries whose answers should not be accessible to users. Such an analysis should take into account not only knowledge that an attacker may have about the mappings, but also what they may know about the semantics of the sources. In this paper, we show that source constraints can have a dramatic impact on disclosure analysis. We study the problem of determining whether a given data integration system discloses a source query to an attacker in the presence of constraints, providing both lower and upper bounds on source-aware disclosure analysis.

==> conc.tex <==
\section{Summary and Conclusion} \label{sec:conc}
We have isolated the complexity of information disclosure from a schema in the presence
of commonly-studied source constraints. A summary of many
combinations of mappings $\M$ and constraints $\sourcecon$ is given
in Table \ref{tab:summary}: 
note that \emph{all problems are complete for the complexity classes
listed}. We have shown tractability for some cases  of bounded arity
and atomic queries, as well as for  $\uid$s and projection maps without restricting queries or arity: these cases
are omitted in the tables. We can also show   that lifting the restrictions in our $\ptime$ results
 leads to intractability (see \cite{fullversion}). But we leave open  a
finer-grained analysis for frontier-one constraints with more general mappings.
\input{table}
Our results depend on a fine-grained analysis of reasoning with TGDs and $\singleconstantrule$s, a topic
we think is of independent interest.




==> reductionwitharitycaveat.tex <==
\section{Reducing Disclosure to Query Entailment} \label{sec:reduction}
Our first goal is to provide a reduction from $\disclose(\sourcecon, \M, \asecretquery)$ to
a finite collection of standard query entailment problems.  %of the form $\qentail(\facts, \Sigma', Q')$. 
For simplicity
we will restrict to Boolean queries $\asecretquery$ in stating the results, but it is straightforward
to extend the reductions and results to the non-Boolean case.
We first recall a prior reduction of $\disclose(\sourcecon, \M, \asecretquery)$ to a more
complex problem, the \emph{hybrid open and closed world query answering problem} 
\cite{hybrid1,hybrid2,hybrid3}, denoted $\hocwq$. $\hocwq$ takes as input a set of facts $\facts$, a collection of constraints $\Sigma$,
a Boolean query $Q$, and additionally a subset of the vocabulary $\closedpreds$.  A \emph{possible world} for
such  $\hocwq(\facts, \Sigma, Q, \closedpreds)$  is any instance $\instance$ containing $\facts$, satisfying $\Sigma$, and such that
for each relation $C \in \closedpreds$, the $C$-facts in $\instance$ are the same as the $C$-facts in $\facts$.
$\hocwq(\facts, \Sigma, Q, \closedpreds)$ holds if $Q$ holds in every possible world. Note that
the query entailment problem is a special case of $\hocwq$, where $\closedpreds$ is empty.

Given a set of mapping rules $m \in \M$ of the form $\phi(\vec y, \vec x) \rightarrow \T(\vec x)$, we let $\globalpreds(\M)$ be the set of global schema predicates, and
let $\viewcon(\M)$ be the mapping rules, considered as bi-directional constraints between global schema
predicates and sources.
%\begin{align*}
%\phi(\vec x, \vec y) \rightarrow \T(\vec x)\\
%\T(\vec x) \rightarrow \exists \vec y \phi(\vec x, \vec y)
%\end{align*}
%We refer to the first as the \emph{forward rule} of $m$ and the second as the \emph{backward rule} of $m$.



We now recall one of the main results of \cite{bbcplics}:

\begin{theorem} \label{thm:critinst} There is an instance $\instance'$ and set of constraints
$\Sigma'$,   computable in linear time from $\sourcecon, \M, \asecretquery$, 
such that  $\disclose(\sourcecon, \M, \asecretquery)$ holds if and only if
$\hocwq(\instance', \sourcecon \cup \viewcon(\M), \asecretquery, \globalpreds(\M))$ holds.
\end{theorem}

In fact, the arguments in \cite{bbcplics} show that 
$\instance'$ can be taken to be a very  simple instance,
the \emph{critical instance} over the global schema $\targetschema$
denoted $\critinst^\targetschema$. The instance mentions only a single element $\critelement$, and contains, for each
relation $R$ in  $\targetschema$ of arity $n$, the fact $R(\critelement, \ldots \critelement)$.
%We write simply $\critinst$ when a schema is understood from context. 


\begin{corollary}  \label{cor:fgtgdupper} $\disclose( \fgtgd, \M, \asecretquery)$
is in $\twoexp$.
\end{corollary}
\begin{proof} 
The non-classical aspect  of $\hocwq$ comes into play with  rules of $\viewcon(\M)$ of  form
$\phi(\vec x, \vec y) \rightarrow \T(\vec x)$. But in the context of  $\critinst$,  these can be rewritten as  \emph{single-constant
 equality rules} ($\singleconstantrule$s)
$\phi(\vec x, \vec y)  \rightarrow \bigwedge_i x_i=\critelement$. Such rules remain in the Guarded Negation Fragment
of first-order logic, which also subsumes $\fgtgd$s, while having a query entailment problem in $\twoexp$ \cite{gnfj}.
%Thus we have exponentially many calls to a $\twoexp$ algorithm, giving the desired $\twoexp$ bound.
\end{proof}




We now want to conduct a finer-grained analysis, looking for cases that give lower complexity.
 To do this we will transform further into a classical query entailment problem. This will require a transformation
of our query $\secretquery$, a transformation of our source constraints and mappings into a new set of constraints,
and a transformation of the instance $\critinst^\targetschema$. The idea of the transformation is that we
remove the $\singleconstantrule$s that are implicit in the $\hocwq$ problem, replacing them with constraints and queries that reflect all the possible
impacts the rules might have on identifying two variables.

We first describe the transformation of the query and the constraints.
They will involve introducing a new unary predicate $\iscrit(x)$; informally
this states that $x$ is equal to $\critelement$.
Consider a CQ $Q=\exists \vec y~ \bigwedge A_i$.
An \emph{annotation} of  $Q$
is a subset  of $Q$'s  variables.
Given an annotation $\annot$ of $Q$, we let $Q_\annot$ be the query
obtained from $Q$ by performing the following operation for
each $v$ in  $\annot$: for all occurrences $j$ of $v$ except the
first one, replacing $v$ with a fresh variable $v_j$; and adding  conjuncts $\iscrit(v_j)$ as well as $\iscrit(v)$ to $Q_\annot$.
A \emph{critical-instance rewriting} of a CQ $Q$ is a CQ obtained by applying the above process to $Q$ for any annotation.
We write $Q_\annot \in \critinstrewrite(Q)$ to indicate that $Q_\annot$ is such a rewriting.

To transform the mapping rules and constraints to a new set of constraints
using $\iscrit(x)$, we lift the notion of critical-instance rewriting to TGDs in the obvious way:
a  critical-instance rewriting of a TGD $\sigma$ (either in $\sourcecon$ or $\viewcon(\M)$),
is the set of  TGDs formed by applying the above process to the body of $\sigma$.
We write
$\sigma_\annot \in \critinstrewrite(\Sigma)$ to indicate that $\sigma_\annot$ is a critical-instance rewriting for a $\sigma \in \Sigma$,
and similarly for mappings. For example, the second mapping rule in Example \ref{ex:simple} has several rewritings;
 one of them will change the rule body 
to   $\patbldg(p,b) \wedge \isopen(b', d) \wedge \iscrit(b) \wedge \iscrit(b')$.


Our transformed constraints will additionally use the set of constraints $\iscrit(\M)$, including all rules:
\[
\T(x_1 \ldots x_n) \rightarrow \iscrit(x_i)
\]
where $\T$ ranges over the global schema and $1 \leq i \leq n$.
Informally $\iscrit(\M)$ states that all elements in the mapping image must be $\critelement$.
We also need to transform the instance,  using a source instance
with ``witnesses for the target facts''.
 Consider a fact $\T(\critelement \ldots \critelement)$ formed by applying
a mapping rule $\bigwedge_i A_i(\vec x_i, \vec y_i) \rightarrow \T(\vec x)$ in $\M$ to $\critinst$.
The \emph{set of witness tuples for $\T(\vec x)$} is the set $A_i(\vec c)$, where $\vec c$ contains
$\critelement$ in each position containing a variable $x_j$ and containing a constant $c_{y_{j}}$ in every
position containing a variable $y_j$.
That is the witness tuples are witnesses for the fact $\T(\critelement \ldots \critelement)$, where each
existential witness is chosen  fresh.
Let $\hide_\M(\critinst^\targetschema)$ be the instance
formed by taking the witness tuples for every fact $\T(\critelement \ldots \critelement)$.
Intuitively, $\hide_\M(\critinst^\targetschema)$ is an instance
very similar to $\critinst^\sourceschema$, but hiding  that  the witnesses
to the existential quantifiers were $\critelement$.






We are now ready to state the reduction of the disclosure problem to query entailment:

\begin{theorem} \label{thm:simplecritinstrewriting} 
$\disclose(\sourcecon, \M, \asecretquery)$ holds exactly when there is a $\secretquery_\annot \in \critinstrewrite(Q)$ such that
$\hide_\M(\critinst)$ entails $\secretquery_\annot$ w.r.t. constraints:
\[
\critinstrewrite(\sourcecon) \cup \critinstrewrite(\M) \cup  \iscrit(\M)
\]
\end{theorem}


Note that  Theorem \ref{thm:simplecritinstrewriting} does not give a polynomial time reduction:
both $\critinstrewrite(\sourcecon)$ and $\critinstrewrite(\M)$ can contain exponentially many rewritings, and further
there can be exponentially many rewritings in $\critinstrewrite(\secretquery)$.

However, the algorithm does  give us a better bound in the case of Guarded TGDs with bounded arity (in our bounded arity
results,  we will always assume a single head atom).

\begin{corollary} \label{cor:gtgdatomicupper} %If  we restrict  each source constraint to be a  $\gtgd$, 
If we bound the  arity of schema relations, then
$\disclose(\gtgd, \guardedmap, \asecretquery)$ is in $\exptime$.
\end{corollary}
\begin{proof}
First, by introducing additional intermediate relations and source
constraints, we can assume that $\M$ contains only projection
mappings.  Thus we can guarantee that $\critinstrewrite(\M)$ just
contains the rules in $\M$.  By introducing intermediate relations and
additional source constraints, we can also assume that each $\gtgd \in
\sourcecon$ has a body with at most two atoms.
%\michael{More detail needed here, as in Louis' write-up or point to appendix} 
Since the arity of relations is fixed, the size of such $1$- or $2$-atom bodies is fixed as well.  From this we see
that the number of constraints in any $\critinstrewrite(\sigma)$ is polynomial. 
The reduction in Theorem \ref{thm:simplecritinstrewriting} thus gives us exponentially many $\gtgd$ entailment problems of polynomial size.
Since entailment over Guarded TGDs with bounded arity is in $\exptime$ \cite{tamingjournal}, we can conclude.
\end{proof}


\subsection{Refinements of the Reduction to Identify Lower Complexity Cases}
In order to lower the complexity to $\exptime$ \emph{without} bounding
the arity, we refine the construction of the function $\critinstrewrite(\sigma)$ in the case where $\sigma$ is a linear TGD, 
providing a function $\critinstrewriteptime(\sigma)$ that constructs only \emph{polynomially many rewritten constraints}.

Let $\sigma=B(\bar{x}) \rightarrow \exists \bar{y} ~ H(\bar{z})$ be
a linear TGD with relation $B$ of arity $k$,  and suppose $\bar{x}$ contains $d$ distinct free variables $V=\{v_1 \ldots v_d\}$.
%We can assume that there is some repetition of variables in $B(\bar{x})$, since otherwise we can proceed as in the ID case.
Let $P$ be the set of pairs $(e,f)$ with  $e < f \leq k$ such that the same variable
$v_i$ sits at positions $e$ and $f$ in $\bar{x}$.
We order $P$ as $(e_0,f_0) \ldots (e_h,f_h)$; for each $(e,f)$ that is not the initial pair $(e_0, f_0)$, we
 let $(e,f)^-$ be its predecessor in the linear order.

 We let $B_{e,f}$ denote new predicates of arity $k$ for each $(e,f) \in P$.
Let $\vec w$ be a set of $k$ distinct variables, and $\vec w^{i=j}$ be formed from $\vec w$ by replacing $w_j$ with $w_i$.
We begin the construction of $\critinstrewriteptime(\sigma)$ with the constraints:

\begin{align*}
B(\vec w^{e_0=f_0}) \rightarrow B_{e_0, f_0}(\vec w^{e_0=f_0})\\
B(\vec w) \wedge \iscrit(w_{e_0}) \wedge \iscrit(w_{f_0}) \rightarrow B_{e_0, f_0}(\vec w)
\end{align*}
We add to $\critinstrewriteptime(\sigma)$ the following constraints, for each $(e,f)$ with a predecessor $(e,f)^-=(e', f')$.
\begin{align*}
  B_{e',f'}(\vec w^{e=f}) \rightarrow B_{e, f}(\vec w^{e=f})\\
B_{e',f'}(\vec w) \wedge \iscrit(w_{e}) \wedge \iscrit(w_{f}) \rightarrow B_{e, f}(\vec w)
\end{align*}
Letting $e_h,f_h$  the final pair in $P$, we add to $\critinstrewriteptime(\sigma)$ the constraint
\[
B_{e_h,f_h}(\vec x') \rightarrow \exists \bar{y} ~ H(\bar{z})
\]
where $\vec x'$ is obtained from $\vec x$ by replacing all but the first
occurrence of each variable $v$  by a fresh variable.
%where $\bar{z}'$ is obtained from $\bar{z}$ by replacing each variable $x_i$ from position
%$i$ of $B(\bar{x})$ with $w_i$.

If $\sourcecon$ consists of $\ltgd$s, we 
let $\critinstrewriteptime(\sourcecon)$ be the result of applying this process to every $\sigma \in \sourcecon$. Similarly,
if $\M$ consists of atomic mappings (implying that the associated  rules  are $\ltgd$s), then
we let $\critinstrewriteptime(\M)$ the result of applying the process above to the  rule going from
source relation to global schema relation associated to  $m \in \M$.
Then we have:




\begin{theorem} \label{thm:fastcritinstrewriting}
$\disclose(\sourcecon, \M, \asecretquery)$ holds exactly when there is a $\secretquery_\annot \in \critinstrewrite(\secretquery)$ such that
$\hide_\M(\critinst)$ entails $\secretquery_\annot$ w.r.t. to the constraints
\[
\critinstrewriteptime(\sourcecon) \cup \critinstrewriteptime(\M) \cup  \iscrit(\M)
\]
\end{theorem}

We can combine this result with recent work on fine-grained complexity  of $\gtgd$s to improve the doubly exponential upper bound
of Corollary \ref{cor:fgtgdupper} for linear TGD source constraints and atomic mappings:


\begin{theorem} \label{thm:linlinupper} 
 %If  we restrict  each source constraint to be an  $\ltgd$ and each mapping to be a atomic, then 
$\disclose(\ltgd, \atomicmap, \asecretquery)$
is in $\exptime$. If the arity of relations in the source schema is bounded, then the complexity drops to $\np$, while
if further the query is atomic, the problem is in $\ptime$.
\end{theorem}

\begin{proof}
It is sufficient to get an $\exptime$ algorithm for the entailment problem produced by Theorem \ref{thm:fastcritinstrewriting}, since
then we can apply it to each $\secretquery_\annot$ in $\exptime$.
The constraints in $\critinstrewriteptime(\sourcecon) \cup \critinstrewriteptime(\M)$ are Guarded TGDs that are not necessarily
$\ltgd$s. 
But the  bodies of these guarded
TGDs consist of a guard predicate and atoms over a  fixed ``side signature'', 
namely the unary predicate $\iscrit$.
It is known that the query entailment
for $\incd$s  and guarded TGDs with a fixed side signature
signature is in {\Exptime}, with the arity dropping to $\np$ (resp. $\ptime$) when the arity is fixed (resp.
fixed and the query is atomic) \cite{antoinemichael}.
\end{proof}

Can we do better than $\exptime$? We  can note that
when the constraints $\sigma \in \sourcecon$ are $\incd$s,  $\critinstrewrite(\sigma)$ consists only of $\sigma$;
similarly if a mapping $m \in \M$ is a projection, then $\critinstrewrite(m)$ consists only of $m$.
This gives us a good upper bound in one of the most basic cases:

\begin{corollary} \label{cor:ididupper} %If  we restrict  each source constraint to be an  $\incd$ and each mapping to be a projection, then
%Problem 
$\disclose(\incd, \projectionmap, \asecretquery)$
is in $\pspace$. If further a bound is fixed on the arity of relations in the source schema, then the problem becomes $\np$, dropping
to $\ptime$ when $\asecretquery$ is atomic.
\end{corollary}
\begin{proof}
Our algorithm will guess a $\secretquery_\annot$ in $\critinstrewrite(Q)$ and checks the entailment  of Theorem \ref{thm:simplecritinstrewriting}.
This gives  an  entailment problem for $\incd$s, known to be in $\pspace$ in general,  in $\np$ for bounded arity,
and in $\ptime$ for bounded arity and atomic queries \cite{johnsonklug}.
\end{proof}

\subsection{Obtaining Tractability}
Thus far we have seen cases where the complexity drops to $\pspace$ in the general case and $\np$ in the bounded
arity case, and $\ptime$ for atomic queries.   We now present a case where we obtain tractability for arbitrary
queries and arity. Recall that a $\uid$ is an $\incd$ where
at most  one variable  is exported. They are are actually quite common, capturing
referential integrity when data is identified by a single attribute. We can show that restricting
to $\uid$s while having only projection maps leads to  tractability:
\begin{theorem} \label{thm:uidptime} %If  we restrict  each source constraint to be an  $\incd$ and each mapping to be a projection, then
$\disclose(\uid, \projectionmap, \asecretquery)$
is in $\ptime$.
\end{theorem}
\begin{proof}
The first step is to  refine the reduction of Theorem~\ref{thm:simplecritinstrewriting} 
to get an entailment problem with only $\uid$s, over an instance consisting of a single
unary fact $\iscrit(\critelement)$. The main issue is  avoid the constraints 
in $\viewcon(\M)$, corresponding to the mapping rules. The intuition for this is that 
on %the input
$\critinst^\targetschema$, the  only impact of the backward and forward implications of $\viewcon(\M)$ 
is  to create new facts  among the source relations.  In
 these new facts only 
% one value, namely 
 $\critelement$, is propagated. 
%By analyzing the schema
%we want to  create new constraints  over the source relations that simulate these compositions to directly generate these facts.
Rather than creating $\singleconstantrule$s (implicitly what happens in the $\hocwq$ reduction) or generating classical constraints
where the impact of the equalities are ``baked in'' (as in the critical-instance rewritings of Theorems \ref{thm:simplecritinstrewriting}
and \ref{thm:fastcritinstrewriting}), we truncate
 the source relations to the positions where non-visible elements occur, while
generating $\uid$s on these truncated relations that simulate the impact of back-and-forth using $\viewcon(\M)$.

The second step is to show that query entailment with $\uid$s over the instance consisting only
of $\iscrit(\critelement)$ is in $\ptime$. This can be seen as an extension of the
$\ptime$  inference algorithm for $\uid$s \cite{uidptimeimp}. The idea behind this result is to analyze
the classical ``chase procedure'' for query entailment with TGDs \cite{faginetaldataex}.
In the case of $\uid$s over a unary fact, the shape of the chase model is very restricted; roughly speaking, 
it is a tree where only a single fact connects two values. Based on this, we can simplify the query
dramatically, making it into an acyclic query where any two variables co-occur in at most one predicate.
Once query simplification  is performed, we can reduce query entailment to polynomial many
entailment problems involving individual atoms in the query. This in turn can be solved using
the $\uid$ inference procedure of \cite{uidptimeimp}.
\end{proof}





==> simpletable.tex <==


\begin{table}[!h]
\resizebox{0.93in}{!}{ 
\begin{tabular}{c|ccccc}
    \backslashbox{$\sourcecon$}{$\M$}                      
     &      $\projectionmap$     & $\atomicmap$ & $\guardedmap$   & CQ Maps    \\ \cline{2-6}
    $\incd$    & \Pspace & \exptimeshort   & \twoexptimeshort   &  \twoexptimeshort \\
    $\ltgd$  & \exptimeshort    & \exptimeshort   & \twoexptimeshort  &  \twoexptimeshort \\
    $\gtgd$  & \twoexptimeshort  & \twoexptimeshort & \twoexptimeshort &   \twoexptimeshort \\
    $\fgtgd$ & \twoexptimeshort  & \twoexptimeshort & \twoexptimeshort   &  \twoexptimeshort \\
\end{tabular}}
\caption{Complexity of disclosure}
\label{tab:gen}
\end{table}

\begin{table}[!h]
\resizebox{0.93in}{!}{ 
\begin{tabular}{c|ccccc}
    \backslashbox{$\sourcecon$}{$\M$}                      
           & $\projectionmap$    & $\atomicmap$ & $\guardedmap$ &  CQ Maps    \\ \cline{2-6}
     $\incd$    & {\NP}    & {\NP}    &   \exptimeshort   &  \twoexptimeshort \\
      $\ltgd$ & {\NP}    & {\NP}    &   \exptimeshort   &  \twoexptimeshort \\
       $\gtgd$  &   \exptimeshort &   \exptimeshort &   \exptimeshort   & \twoexptimeshort \\
        $\fgtgd$ & \twoexptimeshort & \twoexptimeshort & \twoexptimeshort   & \twoexptimeshort \\
\end{tabular}}
\caption{Complexity of disclosure with bounded arity}
\label{tab:bounded}
\end{table}


